Smoothing for age-period-cohort models: a comparison between splines and random process

Age-Period-Cohort (APC) models are well used in the context of modelling health and demographic data to produce smooth estimates of each time trend. When smoothing in the context of APC models, there are two main schools, frequentist using penalised smoothing splines, and Bayesian using random processes with little crossover between them. In this article, we clearly lay out the theoretical link between the two schools, provide examples using simulated and real data to highlight similarities and difference, and help a general APC user understand potentially inaccessible theory from functional analysis. As intuition suggests, both approaches lead to comparable and almost identical in-sample predictions, but random processes within a Bayesian approach might be beneficial for out-of-sample prediction as the sources of uncertainty are captured in a more complete way.

==> documents/manuscript_v1.tex <==
\textbf{Journal: Sociological Methods \& Research}
Timeline: Result there by mid June and writing done 


\section{Introduction}

Important goals for any researcher interested in modelling how disease and/or demographic rates vary over time is the validation of what is driving the underlying phenomena of interest, and forecasting the evolution of rates in the future. Both of these goals work towards the ever important data-driven approach to effective and efficient policy evaluation and recommendation. The class of so-called age-period-cohort (APC) models are a popular tools for modelling the evolution of rates over time when there are different patterns of change by age group. In APC models we consider three time scales: age -- the age of an individual when the event of interest occurs; period -- the time (often year) that the event occurs; and cohort -- the time (usually year) that the individual was born. APC models are often used in a range of health \red{REFERENCES} and sociological \red{REFERENCES} settings.

\red{Paragraph on why prediction is important in general and why APC models can be used}

Although popular, users of APC models must overcome a key technical issue called the `APC Identification Problem'. Because the three time scales of interest are intrinsically connected (e.g., given the the birth year (cohort) and age at event of an individual, we can calculate the year of event (period) as cohort + age), we cannot estimate linear trends along all three time scales simultaneously. A common solution to the identification problem is to parameterise the temporal trends into identifiable quantities which can then modelled using smoothing functions of where there are two main schools: (penalised) splines \red{REFERENCES}, and random processes \red{REFERENCES}. 

It has been shown that smoothing in APC models is essential for the case in which age groups and periods are not given on the same interval width, as otherwise artificial cyclical patterns may appear \citep{holford2006approaches, riebler2010analysis, smith2016review, gascoigne-smith-2023}. Splines are often used for smoothing in a frequentist setting, while random processes, such as random walk models of first or second order, are very common in a Bayesian setting. The choice of implementing APC models in a frequentist or Bayesian setting is often based on philosophical reasons or the background of the applied scientist in charge. In this short report we show that both approaches lead to comparable and almost identical in-sample predictions but that random processes within a Bayesian approach might be beneficial for out-of-sample prediction as the present uncertainty is captured in a more complete way leading to better values of the proper interval score. 

The rest of the article is as follows. In Section 2, we present the England and Wales death due to alcohol and intentional self-harm data and the APC model. In Section 3, we give explain smoothing approaches using penalised splines and random processes and highlight the theoretical link between them. In Sections 4 and 5, we show the exchangeability between the two methods through the use of a simulated data and suicide data. Finally in Section 5, we finish with a discussion.

% \begin{itemize}
%      \item why do people fit APC models
%     \item Why predictions are important (why we use APC models)

%     \item Good models for how disease and demographic rates over time is important to develop or validate hypotheses for drivers of changes in these rates and to plan for the future based on predictions. 
%     \item Age-period-cohort (APC) models are a popular class of tools for modelling the evolution of rates over time when there are different patterns of change by age group. In APC models we consider three time scales: age -- the age of an individual when the event of interest occurs; period -- the time (often year) that the event occurs; and cohort -- the time (usually year) that the individual was born. 
    
%     \item APC models have been used in many sociological and medical applications (reference dump). 
    
%     \item Although popular, users of APC models must overcome a key technical issue called the 'APC Identification Problem'. Because the three time scales of interest are intrinsically connected (e.g., given the the birth year (cohort) and age at event of an individual, we can calculate the year of event (period) as cohort + age), we cannot estimate linear trends along all three time scales simultaneously. 
    
%     \item Lots of people take the approach of focusing on what is estimable within a smoothing framework. Smoothing makes scientific sense (we expect sudden jumps to be very rare) and is a statistically useful device to pool information between observations over different time points when counts of the event of interest are small. 
    
%     \item In this article we explain the connections between two major schools of thought for smoothing that have been used in APC modelling: splines (reference dump) or  random processes (more references).

% \end{itemize}

\section{Age-period-cohort model}\label{sec:apc}

In this article, we consider the application of APC models to mortality from the England and Wales attributed to two underlying causes: mental and behavioural disorders due to use of alcohol (ICD-10 code F10) and (intentional) self-harm (ICD-10 codes X60--X84). The UKs Office for National Statistics (ONS) compiles mortality data from registered deaths by underlying cause, age and time period (week, month, quarter year). We consider counts per year between the years 2006--2021 for 5-year age groups between 25--85. The data from 2013--2021 was extracted through the ONS Nomis tool (https://www.nomisweb.co.uk/) and data from 2006--2012 was assembled from individual annual reports. Mid-year population estimates were extracted by 5-year age group were also extracted for all years form the ONS Nomis tool. In our data, deaths from self-harm are common (insert rate) and deaths from alcohol related disorders are more rare (insert rate)

%https://www.ons.gov.uk/peoplepopulationandcommunity/birthsdeathsandmarriages/deaths/datasets/deathsregisteredinenglandandwalesseriesdrreferencetables

\begin{figure}[!h]
    \centering
    \caption{Suicide deaths due to alcohol (a) and self harm (b) for the years 2006--2021 and ages 24--84. Period is grouped into single years and operates along the $x$-axis. Age is grouped into five-year ages groups and operates along the $y-axis$. Cohort operates along the $y = x$ axis. Deaths are reported as log-rates with the dark-to-light colouring indicating lower-to-higher suicide rates.}
    \label{Fig: ObservedHeatmap_25plus}
    \begin{subfigure}{.5\textwidth}
        \centering
        \caption{Alcohol related deaths}
        \label{Fig: alcoholObservedHeatmap_25plus}
        \includegraphics[width=\linewidth]{alcoholObservedHeatmap_25plus}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \caption{Self harm related deaths}
        \label{Fig: selfHarmObservedHeatmap_25plus}
        \includegraphics[width=\linewidth]{selfHarmObservedHeatmap_25plus}
    \end{subfigure}
\end{figure}

Figure \ref{Fig: ObservedHeatmap_25plus} shows the age-specific rates over time for the two causes of death. The natural logarithmic are the rates are shown to allow a closer inspection of the trends in age, period and cohort. An extra $1/2$ event is added to each mortality count to avoid taking logs of $0$. For both causes we see there is substantial variation in risk according to age and some evidence of trends over year of death. \red{EXAMPLES}

There are also age by year interactions -- which could indicate cohort effects. For example, there is a big increase in self harm mortality in the youngest age groups from 2019--2021 that is not seen in the older age groups. This could be a result of a change in reporting or a genuine increase in self harm rates in more recent birth cohorts.  

A traditional APC model that is used to capture expected incidence rates as a log-linear model contains additive functions of age, period and cohort. Due to the identification issues (cohort = period - age), the temporal linear trends are unidentifiable and APC models are often reparameterised. One such reparameterisation is in terms of identifiable curvature functions that are orthogonal to their respective linear trends \citep{holford1983estimation}. For ages $a = 1, \dots A$ and period $p = 1, \dots, P$, we define an APC model in terms temporal curvature functions,
\begin{equation}
	\label{Eq: APC model}
	\lambda_{ap} = \beta_0 + \beta_1{s_a} + \beta_2{s_p} + \ageCurv\pa{a} + \perCurv\pa{p} + \cohCurv\pa{c}
\end{equation}
where $\lambda_{ap} = \log\pa{\EE\bra{y_{ap}/N_{ap}}}$ is the log of the expected rate, and $\ageCurv, \perCurv$ and $\cohCurv$ are the age, period and cohort functions of curvature. The reparameterisation implicitly assumes the effect of the cohort effect is zero; therefore, the terms ${s_a}$ and ${s_p}$ are interpreted as the age + cohort and period + cohort slopes. In this article, we focus on estimates and predictions of the linear predictor, $\lambda_{ap}$, which is always identifiable. Consequently, the choice of reparameterisation becomes less important; however, when using APC models, it has been recommended to always start with an identifiable model \citep{smith2016review}. 

% A (continuous) age-period-cohort (APC) model for  that captures all three temporal trends is,
% \begin{equation}
% 	\label{Eq: Unidentifiable APC model}
% 	g\pa{\mu_{ap}} = \linPred_{ap} = \ageFull\pa{a} + \perFull\pa{p} + \cohFull\pa{c}
% \end{equation}
% where $g\pa{\cdot}$ is the link function, $\mu_{ap} \equiv \EE\bra{y_{ap}}$ is equivalent to the expected value of the response, $\linPred_{ap}$ is the linear predictor and $\ageFull$, $\perFull$ and $\cohFull$ are the smooth functions of age $a$, period $p$ and cohort $c$. The observations $y_{ap}$ are modelled as observations of a random variable with the probability density (likelihood) function $\mL\pa{\bs{f},\bs{\theta}} = \pi\pa{\bs{y} | \bs{\mu}, \bs{\theta}}$ where $\bs{\theta}$ is a vector of additional parameters in the likelihood (i.e., the variance).

% {\color{violet} Should we just start straight away with Poisson here to keep things concrete, and maybe mention the more general link/likelihood after? Could also introduce the APC model after the data}
% \blue{CG: like this idea}

For health and sociological data that comes aggregated in equal bins (i.e., age and period both single-year), the curvature terms are identifiable However, when APC models are fit to data such as in Figure \ref{Fig: ObservedHeatmap_25plus}, where the temporal groups are aggregated in unequal bins (i.e., age is aggregated into five-years rather than the single-years of period), there curvature terms become unidentifiable and display a cyclic pattern as a result \citep{holford2006approaches, riebler2010analysis}. To ensure the model is robust at alleviating any additional identification problems related to non-equal binning of the data, it is recommended to include a penalty on the second derivatives of the curvature terms \citep{gascoigne-smith-2023}.

\section{Smoothing approaches}

% To describe smoothing in both a frequentest and Bayesian framework, we will use a simple one-dimensional model for smoothing a response variable,
% \begin{equation}
%     \label{Eq: Simple Univariate Nonparametric Model}
%     y_i = f\pa{x_i} + \epsilon_i \qquad i = 1, \dots, n 
% \end{equation}
% where $y_i$ are observations, $f$ is a smooth function of the covariate $x_i$ that is unknown and we wish to estimate, and $\epsilon_i \sim \text{N}\pa{0, \sigma^2}$ is an unstructured random (measurement) error. The observations are modelled as an observation of a random variable with the probability density (likelihood) function $\mL\pa{\bs{f},\bs{\theta}} = \pi\pa{\bs{y} | \bs{\mu}, \bs{\theta}}$ where $\mu_i$ is the location parameter (i.e., $\EE\pa{y_i}$) and $\bs{\theta}$ is a vector of additional parameters in the likelihood (i.e., the variance). Currently, we consider our observations to be Gaussian but this can be extended to consider non-Gaussian observations using a link function, $g$, so the response is modelled with a specific distribution with the mean $g^{-1}\pa{f\pa{x}}$.

\subsection{Smoothing splines}

For the purpose of explanation, we describe smoothing for a simple univariate function. Consider the age component in the APC model presented in Section \ref{sec:apc}, $g\pa{\mu_a} = \ageFull\pa{a}$. In a frequentist paradigm, an estimator of $f$ can be found by maximising the following penalised log-likelihood,
\begin{equation}
    \label{Eq: Cubic Penalised Log-Likelihood}
    \widehat{\ageFull}, \hat{\theta} = \argmax_{\ageFull, \theta} l\pa{\ageFullB, \bs{\theta}} +  \lambda \int \ageFull''\pa{a}^2 d{a}
\end{equation}
where $l\pa{\ageFullB, \bs{\theta}} = \log\mL\pa{\ageFullB,\bs{\theta}}$ is the log-likelihood, and  $\int \ageFull''\pa{a}^2 d{a}$ is a penalty function on the second derivative of the smooth function $\ageFull$ with smoothing parameter $\lambda$ that controls the trade-off between model fit and smoothness. The inclusion of the penalty function on the second derivative of $\ageFull$ penalises $\ageFull$ when it deviates from linearity. If $\lambda = 0$, there is no cost for fitting complicated functions and $\widehat{\ageFull}$ can be extremely `wiggly'. As $\lambda \rightarrow \infty$, the cost for fitting a complicated function increases and $\widehat{\ageFull}$ is forced to be closer to linearity. 

When maximising Equation \ref{Eq: Cubic Penalised Log-Likelihood}, the true functions $f$ needs a finite basis approximation. It is common in sociological and health settings to use a spline basis to approximate the true function $\ageFull$ when maximising the penalised log-likelihood \citep{heuer1997modeling, holford2006approaches, carstensen2007age}. A spline basis is a set of polynomial (basis) functions which are based on points called knots. Given $b_k\pa{x}$, the $k^\text{th}$ basis function, $f$ is approximated with a spline as follows
\begin{equation*}
    \label{Eq: Basis Approximation For f}
    \ageFull\pa{a} = \sum_{k = 1}^{K} b_{k}\pa{a} \beta_{k} = \bs{X}\bs{\beta}
\end{equation*}
where $K$ is the number of basis function, $\beta_{k}$ are the unknown weights to be estimated and $\bs{X}$ is an $n \times K$ matrix of basis vectors. With this basis representation, the penalty function for $\ageFull$ can be rewritten
\begin{equation*}
    \label{Eq: Basis Approximation For Cubic Penalty}
    \int \ageFull''\pa{a}^2 d{a} = \bs{\beta} \int \bs{b}^T\pa{a}\bs{b}\pa{a} d{a} \bs{\beta} = \bs{\beta} \bs{S} \bs{\beta}
\end{equation*}
where $\bs{S} = \int \bs{b}^T\pa{a}\bs{b}\pa{a} d{a}$ is known as the penalty matrix. Therefore, the penalised log-likelihood to be maximised can be re-written in terms of the finite basis approximation to each of the smooth functions,
\begin{equation}
    \label{Eq: Basis Approximation For Cubic Penalised Log-Likelihood}
    l_p\pa{\bs{\beta}, \bs{\theta}} = l\pa{\bs{\beta}, \bs{\theta}} + \lambda \bs{\beta} \bs{S} \bs{\beta}.
\end{equation}
where $l_p\pa{\bs{\beta}, \bs{\theta}} = \log\mL_p\pa{\bs{\beta}, \bs{\theta}}$ is the penalised log-likelihood that is maximised by $\hat{\bs{\beta}}$ and $\hat{\bs{\theta}}$. Smoothing splines within the context of APC models have been used besides others by \citet{carstensen2007age, fu2008,jiang2014}.

An important aspect of fitting splines is defining how many knots to use and where to place them. The more knots, the more flexible the spline is, but without a penalty this can lead to over fitting. Using a toy dataset, Figure \ref{Fig: whyIncludePenalty} highlights how a penalty reduces the importance of nuance when choosing the number of knots. In the toy data set, the number of unique ages was $A = 15$. We used three knots to define the low-knots. Three is the minimum number of knots we could use to ensure the second derivatives are continuous and can be penalised. We used 15 knots to define the high-knots. High-knots without a penalty clearly overfits. High-knots with a penalty is a smooth curve similar to that of low knots. The inclusion of the penalty ensures no overfitting whilst maximising the amount of information to be gained by including more knots.

\begin{figure}[!h]
    \centering
    \caption{Example of how a penalty on the second derivatives of the basis functions used to define a spline model ensures over fitting does not occur. The red and green curves are fit using a basis with a low knots number of knots and the blue and purple curves are with a high number of knots. The red and blue include a penalty term on the second derivatives of the basis functions and the green and purple terms do not.}
    \label{Fig: whyIncludePenalty}
    \includegraphics[width=0.5\textwidth]{whyIncludePenalty}
\end{figure}

\subsection{Random processes}

%We use Gaussian Markov random fields (GMRFs) for smoothing in a Bayesian paradigm. For convenience of notation, let $f_i = f\pa{x_i}$; consequently, a vector $\bs{f} = \{f_1, \dots, f_n\}$ is called a GMRF with mean $\bs{\mu}$ and precision $\bs{Q}$ if it has a density of the form
%\begin{equation}
%    \label{Eq: General GMRF}
%    \pi\pa{\bs{f}} = \frac{1}{\pa{2\pi}^{n/2}}\abs{\bs{Q}}^{1/2}\exp\pa{-\frac{1}{2}\pa{\bs{f} - \bs{\mu}}^T \bs{Q}\pa{\bs{f} - \bs{\mu}}}
%\end{equation}
%where $\bs{Q}$ is positive definite and holds for the following conditional %independence (Markov) property,
%\begin{equation*}
%    \label{Eq: Sparse Q Conditional Independence Property}
%    f_i \perp f_j | \bs{f}_{-ij} \Longleftrightarrow Q_{ij} = 0
%\end{equation*}
%where $\bs{f}_{-ij}$ are all elements in $\bs{f}$ without $f_{ij}$ and $i \neq j$. \cite{rue2005gaussian} Due to the conditional independence, most of the entries in the precision matrix $\bs{Q}$ are zero with only a few being non-zero, this means $\bs{Q}$ is a sparse matrix. Sparsity of a matrix is an important property as it offers excellent computational advantages over non-sparse (dense) matrices. Consider $\bs{Q}$ to be an $n \times n$ precision matrix. When $\bs{Q}$ is sparse, the order of the cost for any computations (such as inference) using $\bs{Q}$ is $\mO\pa{n^{3/2}}$. For the corresponding dense $\bs{Q}^{-1}$, the same computational costs are of order $\mO\pa{n^3}$. \cite{bakka2018spatial}

In a Bayesian paradigm, random processes are commonly used for smoothing. For temporal smoothing in sociological and health contexts, random walks of order 1 and 2 (RW1 and RW2, respectively) are very popular, so that they are also widely used within APC models for both estimation and prediction \citep{berzuini1993bayesian, berzuini1994bayesian, besag1995bayesian,  knorr2001projections, riebler2010analysis, riebler2012estimation, riebler2016intuitive, cameron2021}. \citet{okui2021} used random walk priors in an APC model to analyze the prevalence of common psychiatric disorders in Japan. The popularity of both the RW1 and RW2 models is not only due to their smoothing properties with RW1 and RW2 models smoothing by penalising deviations in the constant and linear trends, respectively, but as they are (intrinsic) Gaussian Markov random fields (GMRFs) with sparse inverse covariance matrices, i.e.\,precision matrices, they offer good computational properties. 

Similarly to the penalised smoothing splines, a RW2 penalises deviations in linearity \cite{rue2005gaussian}. Assuming $\ageFullB$ follows a RW2 model, the second differences have the distribution
\begin{equation*}
    \label{Eq: Second Difference Distribution for RW2}
    \Delta^2 {\ageFull}_i \sim_\text{iid} \text{N}\pa{0, \tau^{-1}}
\end{equation*}
where $\tau$ is the inverse variance parameter called precision parameter. The precision $\tau$ controls the trade-off between smoothness and closeness to the data (it is the smoothing parameter), and has parallels with the smoothing parameter $\lambda$ in the GAM framework; for example, $\tau \rightarrow \infty$ shrinks the distribution towards the mean whilst $\lambda \rightarrow \infty$ smooths towards the mean. The joint density of $\ageFullB$ is defined, 
\begin{equation}
    \label{Eq: Joint Density of the RW2}
    \begin{split}
        \pi\pa{\ageFullB | \tau} & \propto \tau^{{\pa{n - 2}}/{2}} \exp \pa{-\frac{\tau}{2} \sum_{i = 1}^{n - 2} \pa{ {\ageFull}_i - 2{\ageFull}_{i+1} + {\ageFull}_{i+2} }^2 } \\
        & = \tau^{{\pa{n - 2}}/{2}} \exp \pa{ \frac{1}{2} \ageFullB^T \bs{Q} \ageFullB }
    \end{split}
\end{equation}
%which has the conditional mean and precision
%\begin{equation*}
%    \label{Eq: RW2 Mean and Varaince}
%    \begin{split}
%        \EE\pa{f_i | \bs{f}_i, \tau} & = \frac{4}{6} \pa{f_{i+1} + f_{i-1}} - \frac{1}{6} \pa{f_{i+2} + f_{i-2}} \\
%        \text{Prec}\pa{f_i | \bs{f}_i, \tau} & = 6 \tau
%    \end{split}
%\end{equation*}
%respectively for $2 < i < n-2$. 
with precision matrix %for a RW2 has the form
\begin{equation*}
    \label{Eq: RW2 Precision}
    \bs{Q} = \tau \bs{R} = \tau
    \begin{pmatrix*}[r]
        1 & -2 & 1 \\
        -2 & 5 & -4 & 1 \\
        1 & -4 & 6 & -4 & 1 \\
        & \ddots & \ddots & \ddots & \ddots & \ddots \\
        & & 1 & -4 & 6 & -4 & 1 \\
        & & & 1 & -4 & 5 & -2 \\
        & & & & 1 & -2 & 1 \\
    \end{pmatrix*}
\end{equation*}
where $\bs{R}$ is referred to as the structure matrix. Due to the Markov property, the RW2 precision matrix is of rank $n-2$ and is rank deficient, so that the RW2 is an improper or intrinisic GMRF. Of note, the definition of the RW1 is based on the first differences and analogous to the defintion of the the RW2, for details we refer to \citet[Section 3.3.1]{rue2005gaussian}. %Therefore, Equation \eqref{Eq: Joint Density of the RW2} is technically not a proper distribution meaning it is no longer a GMRF, but an improper GMRF. In general, a RW of order $p$ model is an improper GMRF with the precision matrix being of rank $n-p$.

\subsection{Connections between penalised smoothing splines and random processes}

There are theoretical parallels between estimates produced from penalised smoothing spline models and random walk models based on theory from functional analysis. We wish to identify the key information from this theory so that a general practitioner can make the connection and use the methods interchangeably. When estimating $\ageFull$, we have shown above that we can either define a finite dimensional approximation to $\ageFull$ and then estimate the parameters of the approximation by maximising the penalised log-likelihood or we can place a prior on $\ageFull$ and define estimates of the model parameters by evaluating the posterior distribution via Bayes rule.

% By taking a partially informative Gaussian process prior on the function $f$, \cite{kimeldorf1970correspondence}, and later formalised by \cite{wahba1978improper}, identified a correspondence between random processes and a penalised smoothing splines. The penalised log-likelihood estimator of Equation \eqref{Eq: Simple Univariate Nonparametric Model} is one that maximises
% \begin{equation*}
%     \label{Eq: Generic Penalised Log Likihood Estimator}
%     \hat{f}, \hat{\theta} = \argmax_{f, \theta} l\pa{\ageFullB, \bs{\theta}} +  \lambda \int f^{\pa{p}}\pa{x}^2 d{x}
% \end{equation*}
% where $\int f^{\pa{p}}\pa{x}^2dx$ is a order-$p$ penalty for the smooth $f$ with the smoother parameter $\lambda$. For the cubic penalty, $p = 2$. A partially informative Gaussian process prior on $f$ is of the form,
% \begin{equation*}
%     \label{Eq: Partially Informative Prior}
%     \beta_0 + \beta_1 x + \dots + \beta_{p-1} x^{p-1} + \delta^\frac{1}{2}Z\pa{x}
% \end{equation*}
% where $\beta_0, \dots, \beta_{p-1} \sim \text{N} \pa{0, \xi}$ as $\xi \rightarrow \infty$ which is ``diffuse'' (flat) on the coefficients that span the null space of the penalty (for a cubic penalty, this is the constant and linear terms) and ``proper'' for the Gaussian process $Z\pa{x}$ and $\delta$ is a scale parameter. \cite{wahba1978improper} showed that the polynomial smoothing spline that maximises the penalised log-likelihood, $\hat{f}$, is equivalent to Bayesian estimation with a partially informative Gaussian process prior on $f$,
% \begin{equation*}
%     \label{Eq: Wahbas Result}
%     \hat{f} = \lim_{\xi \rightarrow \infty}\EE_{\xi}\bra{p\pa{f} | \bs{y}}
% \end{equation*}
% where $\xi \rightarrow \infty$ corresponds to the ``diffuse'' part of the prior. Therefore, the correspondence is between the polynomial smoothing spline maximiser of the penalised log-likelihood and the posterior expectation of the Gaussian random field defined by a partially informative Gaussian process prior. This result was later extended by \cite{speckman2003fully}, who showed the class of priors that are appropriate for the correspondence includes those motivated by a difference approximation in the penalty for the penalised smoothing splines. 

% \textcolor{red}{Andrea: Maybe ok to start here and only summarize the part above?}
% \blue{CG: See you have done this Andrea so commenting out}

To see the relation between a penalised smoothing spline and RW2 prior model, lets rewrite the penalised log-likelihood in Equation \eqref{Eq: Basis Approximation For Cubic Penalised Log-Likelihood} in terms of a likelihood,
\begin{equation*}
    \label{Eq: Cubic Penalised Likelihood}
    \mL_p\pa{\bs{\beta}, \bs{\theta}} = \mL\pa{\bs{\beta}, \bs{\theta}} \times \exp\pa{- \lambda \bs{\beta}^T \bs{S} \bs{\beta}}.
\end{equation*}
If we consider the key concept in Bayesian inference ($posterior \propto prior \times likelihood$), $\mL_p\pa{\bs{\beta}, \bs{\theta}}$ and $\mL\pa{\bs{\beta}, \bs{\theta}}$ are equivalent to the posterior distribution and the likelihood function, respectively and $\exp\pa{- \lambda \bs{\beta}^T \bs{S} \bs{\beta}}$ can be thought of as the prior distribution of the parameters $\bs{\beta}$. The prior distribution
\begin{equation*}
    \label{Eq: Prior Distribution From Penalised Likelihood}
    p\pa{\bs{\beta} | \lambda} \propto \exp\pa{- \bs{\beta}^T \bs{Q}_\lambda \bs{\beta}}
\end{equation*}
where $\bs{Q}_\lambda = \lambda \bs{S}$ is of the form of an improper GMRF prior on a regular lattice \citep{wood2006generalized, yue2012priors}. The impropriety in the prior is due to the penalty matrix $\bs{S}$ not being of full rank, meaning the precision matrix $\bs{Q}_{\lambda}$ is not invertible. The precision matrix is rank deficient by the dimension of the null space for the penalty matrix $\bs{S}$. A random walk of order $p$ prior is an improper Gaussian prior (with a Markov property) which has a rank deficiency of $p$. If we choose to use a RW2 prior, then $\bs{Q}_\lambda$ will be an improper GMRF with a rank deficiency of two. This is equivalent to using the cubic penalty function since $\bs{S}$ is rank deficient by two. Because of this, both the RW2 prior and the penalty are penalising deviations in linearity. 

Whilst both the penalised smoothing spline model and the RW2 prior model are imposing a penalty on the second derivative of the estimates, how each model performs this differs which causes slight differences in practical estimates. For example, the smoothing parameter of the penalised smoothing spline model is estimated by cross validation \citep{wood2006generalized} in \mgcv\, whereas the equivalent smoothing parameter of the RW2 prior model in \inla \ is based upon the choice of the prior distribution \cite{rue2005gaussian}. The data driven approach of the penalised smoothing spline model is attempting to find an `optimal’ smoothing parameter; whereas in the RW2 prior model, we specify a distribution for the smoothing parameter \textit{a priori}.

As recommended by \citet{simpson2017penalising} we put a penalised complexity (PC) prior for the smoothing parameter $\tau$, which is a type-2 Gumbel distribution for $\tau$ or equivalently an exponential distribution on the standard deviation $\sigma= \sqrt{1/\tau}$ with parameter $\theta$. The rate parameter $\theta$ is chosen based on a probability contrast for $\sigma$, specifying $\text{Prob}(\sigma >U) = \alpha$, with $U>0$ and $\alpha \in (0,1)$, such that $\theta = -\ln(\alpha)/U$. For details, we refer to \citet{simpson2017penalising}. Figure \ref{Fig: pcPriorsPlot} shows the three PC priors we will consider in the following, using $\alpha=0.01$ and either $U=1$, $U=3$ or $U = 6$.

\begin{figure}[!h]
    \centering
    \caption{The two types of PC priors we use for the random processes, shown for the standard deviation $\sqrt{1/\tau}$. The red curve uses $U = 1$, and the blue curve has $U = 3$. For both, $\alpha = 0.01$.}
    \label{Fig: pcPriorsPlot}
    \includegraphics[width=0.5\textwidth]{pcPriorsPlot}
\end{figure}

% \textcolor{red}{AR: might be better two used two different gray scales or dashed vs. solid lines. I guess the legend can be omitted. Add y-axis label and make tickmarks bigger} -  CG: have changed the line types, will need to increase the text size once we are happy 


\section{Simulation study} \label{Section: Simulation Study}

The simulation study is motivated by the the alcohol related deaths from Section \ref{sec:apc}. The shapes for the age, period and cohort effects are adopted from a simulation study for Gaussian data from Luo and Hodges \citep{luo2016block}. To keep the shapes of the age, period and cohort functions, but make the responses representable for the low-count alcohol related death, we included a scale and shift alongside the functions of \cite{luo2016block}. A similar alteration was performed in \cite{gascoigne-smith-2023}. 

We generated observations using single-year ages (from 10--84) and periods (2000--2020). We fixed 750\,000 as the population at risk for each age-period combination motivated by \red{cite here for this value}. To mimic the reality of data collection and dissemination, we generated data in single year age-period combinations and then aggregated age into five-year groups, i.e., $10 - 14, 15 - 19, \dots, 80 - 84$. When modelling, we used the midpoint of the ages groups, i.e., $12.5, 17.5, \dots, 82.5$. We simulated $k = 1, \dots, K = 100$ data sets in this way. For each data set we assess both the estimation and predictive capabilities. We fit the model for all years between 2000--2017 and forecast for years 2018--2020. 

For the simulation study, we used three common spline basis functions, Cubic Regression Splines (CRS), B-Splines (BS) and Thin Plate Regression Splines (TPRS). For details, we refer to \cite[Chapter 5;][]{wood2006generalized}. The results in Figure \ref{Fig: whyIncludePenalty} show the choice of the number of knots to use becomes less important when including a penalty as it ensures there is no over-fitting. Consequently, we use 10, 10 and 12 for the number of age, period and cohort knots, respectively, when defining their basis functions. We fit a RW2 model with three different PC prior specifications. For all specifications, we used $\alpha = 0.01$ and either $U = 1$, $U = 3$ or $U = 6$.

\subsection{Assessment criteria}

We assessed the models estimation and prediction performance using the Mean Absolute Error (MAE) and Mean Square Error (MSE) computed separately for the estimation and in-sample prediction. We defined the MAE and MSE,
\begin{equation*}
    \label{Eq: MAE and MSE}
    \text{MAE}_{ap} = \frac{1}{K} \sum_{k=1}^{K} \abs{\hat{\lambda}_{ap} - \lambda_{ap}} \quad \text{and} \quad \text{MSE}_{ap} = \frac{1}{K} \sum_{k=1}^{K} \pa{\hat{\lambda}_{ap} - \lambda_{ap}}^2
\end{equation*}
where for age $a$ and period $p$, $\hat{\lambda}_{ap}$ and $\lambda_{ap}$ are the fitted and true log-rates, respectively.

In addition to the MAE and MSE, we assessed the entire predictive distribution using the 95\% Interval Score (IS) \citep{gneiting2007strictly}. The IS is a scoring rule that transforms interval width and empirical coverage into a single score. Let $\lambda_{ap}$ be the true log-rate for age $a$ and period $p$ with an associated lower and upper uncertainty, $\bra{l_{ap}, u_{ap}}$, defined using the respective $\pa{1 - \alpha} \cdot 100 \%$ lower and upper predictive quantiles. The IS for $\alpha \in \pa{0,1}$ is defined 
\begin{equation*}
    \label{Eq: Interval Score}
    \text{IS}_{\alpha}\pa{\lambda_{ap}} = \pa{u_{ap} - l_{ap}} + \frac{2}{\alpha}\pa{l_{ap} - \lambda_{ap}}\II\bra{\lambda_{ap} < l_{ap}} + \frac{2}{\alpha}\pa{\lambda_{ap} - u_{ap}}\II\bra{\lambda_{ap} > u_{ap}}
\end{equation*}
where $\II\bra{\cdot}$ is an indicator function that penalises how many data points are outside the interval. The final score is defined by averaging over all IS's, $\text{IS}_{\alpha} = \Sigma_{ap} \text{IS}_{\alpha}\pa{\lambda_{ap}}$. A lower IS is indicative of a better performing model. We also considered the interval width and the coverage.   

\subsection{Implementation}

We fitted the penalised spline model model with the Generalised Additive Model (GAM) framework, as implemented in the \mgcv \ package \citep{wood2006generalized}. \mgcv \ offers a wide range of spline bases to represent smooth functions and their penalties. In \mgcv, the syntax to fit a penalised TPRS on the term \texttt{x} is \texttt{s(x, bs = `tprs', k = k)}. The argument \texttt{bs = `tprs'} defines the type of basis function function (TPRS), and the argument $\texttt{k}$ is for the number of knots used to defined the basis. 

We fitted the RW2 model within a Bayesian hierarchical framework using Integrated Nested Laplace Approximation (INLA), as implemented in the \inla \ package \citep{rue2009approximate}. INLA provides accurate approximations of the marginal posterior distribution for all model parameters whilst avoiding the need for costly and time-consuming Markov-chain Monte Carlo (MCMC) sampling. In \inla, the syntax to fit a RW2 prior on the term \texttt{x} is \texttt{f(x, model = `rw2', ...)}. The only argument that needs to be explicitly defined to fit a RW2 prior model is \texttt{model = `rw2'}. Other additional arguments that are commonly used are:  $\texttt{extraconstr = list(A, e)}$ where $\texttt{A} = \bs{C}$ is the constraint matrix and $\texttt{e} = \bs{0}$ to specify the constraint explicitly, and \texttt{hyper} for the specification of the prior specification.

\subsection{Results}

\begin{figure}[!h]
    \centering
    \caption{Boxplots for Mean Absolute Error (a) and Mean Square Error (b) for the simulation study. Each boxplot is split into two facets, one facet comparing the estimated values against the true values (left), and the other comparing the in-sample prediction values against the true values (right). In each facet, the first three boxes are spline models defined with Cubic Regression Splines (CRS), B-Spline (BS) and Thin Plate Regression Spline (TPRS) basis. The last three boxes are Random Walk 2 models define using $U = 1, 2$ and $6$ in the Penalised Complexity priors.}
    \label{Fig: boxplots}
    \begin{subfigure}{.49\textwidth}
        \centering
        \caption{Mean Absolute Error}
        \includegraphics[width=\linewidth]{maeBP}
    \end{subfigure}%
    \begin{subfigure}{.49\textwidth}
        \centering
        \caption{Mean Square Error}
        \label{Fig: mseBP}
        \includegraphics[width=\linewidth]{mseBP}
    \end{subfigure}
\end{figure}

Figure \ref{Fig: boxplots} shows the boxplots the MAE and MSE for the different models. First consider the results for the estimated values. Within the spline models, the results are robust to the choice of the basis functions used. The same is true for within the RW2 models for the different specification of priors. Comparing between the spline and RW2 models, the spline models performed slightly better when estimating with the box plots being closer to zero for both scores. This difference is due to the difference in how each approach estimates the smoothing parameter. The smoothing parameter for the penalised smoothing spline is the optimal parameter found through cross-validation, whereas the smoothing parameter in the RW2 model is defined \textit{a-prior} and can over-smooth in comparison to the optimal parameter. As the data has unequal age and period intervals, the period and cohort functions will incur a larger penalty \citep{gascoigne-smith-2023}; consequently, any difference in the estimation of the smoothing parameter are exacerbated. 

For the in-sample prediction, the results are robust against the prior specification, but not the basis specification. The TPRS had a lower MAE and MSE than the both of the CRS and BS bases. Similarly to why the penalised smoothing splines outperformed the RW2 model, the TPRS performed better in predictions as is is known as an optimal smoothing basis for any given basis \citep{wood2003thin}. For both set of results, the differences within each method and between the methods is small when considering the scales of the MAE and MSE, $\times 10^{-2}$ and $\times 10^{-3}$, respectively. 

Each set of simulated data produced its own IS, interval width and coverage for each model. We averaged these over all simulations and the results are in Table \ref{Tab: Simulation Study Model Scores}. The thin-plate regression spline and the $U = 1$ specification of the spline and RW2 models were the best performing models from each (for both estimation and in-sample prediction) in terms of IS. The thin plate regression spline was the best performing overall. The small relative difference within the penalised smoothing spline and RW2 models provided evidence of the robustness to basis and prior specification. The penalised smoothing spline models out performed the RW2 models, but this is due to the method of estimating the smoothing parameters. Overall, the differences between the two approaches is relatively small and it is feasible to use the penalised smoothing spline and RW2 models interchangeably.

\begin{table}[!h]
    \centering
    \caption{Model scores for the simulation study. The First three rows are for the spline models and the latter three rows are for the random walk 2 models. The columns are split into scores for estimation and the in-sample prediction. Each simulation study has its own score, and the values are the average over all simulations.}
    \label{Tab: Simulation Study Model Scores}
    \resizebox{\textwidth}{!}{%
        \begin{tabular}{|c|c|ccc|ccc|}
            \hline
            \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\ Type\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\ Specification\end{tabular}}} & \multicolumn{3}{c|}{\textbf{Estimation}} & \multicolumn{3}{c|}{\textbf{In-Sample Prediction}} \\ \cline{3-8} 
            &  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Interval Score}\\ $\pa{\times 10^{2}}$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Interval width}\\ $\pa{\times 10^{2}}$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{Coverage}\\ (\%)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Interval Score}\\ $\pa{\times 10^{2}}$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Interval width}\\ $\pa{\times 10^{2}}$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{Coverage}\\ (\%)\end{tabular} \\ \hline
            \multirow{3}{*}{\textbf{Spline}} & Cubic regression & \multicolumn{1}{c|}{13.33} & \multicolumn{1}{c|}{10.82} & 94.32 & \multicolumn{1}{c|}{25.60} & \multicolumn{1}{c|}{16.10} & 88.00 \\ \cline{2-8}
            & B-spline & \multicolumn{1}{c|}{13.37} & \multicolumn{1}{c|}{10.76} & 94.07 & \multicolumn{1}{c|}{25.80} & \multicolumn{1}{c|}{16.30} & 87.82 \\ \cline{2-8} 
            & Thin-plate regression& \multicolumn{1}{c|}{13.23} & \multicolumn{1}{c|}{10.80} & 94.45 & \multicolumn{1}{c|}{25.40} & \multicolumn{1}{c|}{15.96} & 88.16 \\ \hline
            \multirow{3}{*}{\textbf{Random Walk 2}} & $\alpha = 0.01$ \& $U = 1$ & \multicolumn{1}{c|}{15.18} & \multicolumn{1}{c|}{14.22} & 97.64 & \multicolumn{1}{c|}{32.31} & \multicolumn{1}{c|}{32.09} & 99.60 \\ \cline{2-8} 
            & $\alpha = 0.01$ \& $U = 3$ & \multicolumn{1}{c|}{15.26} & \multicolumn{1}{c|}{14.31} & 97.67 & \multicolumn{1}{c|}{32.79} & \multicolumn{1}{c|}{32.58} & 99.62 \\ \cline{2-8} 
            & $\alpha = 0.01$ \& $U = 6$ & \multicolumn{1}{c|}{15.28} & \multicolumn{1}{c|}{14.33} & 97.69 & \multicolumn{1}{c|}{32.90} & \multicolumn{1}{c|}{32.69} & 99.62 \\ \hline
        \end{tabular}%
    }
\end{table}


\section{Illustration: death due to alcohol and intentional self-harm}

Figure \ref{Fig: Predicted_splineVsRW2} shows the fitted values for the spline and RW2 models for the two outcomes. In each scenario, both sets of estimated and predicted values fall along the $y = x$ axis, hence are similar to one another. To quantify the performance of each model, the models scores, as defined in Section \ref{Section: Simulation Study}, for each model on each data set are in Table \ref{Tab: Suicide data model fit Scores}. In all cases (data set, model type and whether estimation or prediction), the spline model was the best performer with the lowest interval score. 

\begin{figure}[!h]
    \centering
    \caption{Comparison of the estimated and in-sample predicted alcohol (a) and self harm (b) related suicide values from the spline and random walk 2 model. In each subfigure, the spline values are along the $x$-axis and the random walk 2 values are on the $y$-axis. The red dotted line is the $y=x$ axis. The green circles and blue triangles represent the estimated and predicted values, respectively.}
    \label{Fig: Predicted_splineVsRW2}
    \begin{subfigure}{.49\textwidth}
        \centering
        \caption{Alcohol related deaths}
        \label{Fig: alcoholPredicted_splineVsRW2}
        \includegraphics[width=\linewidth]{alcoholPredicted_splineVsRW2}
    \end{subfigure}%
    \begin{subfigure}{.49\textwidth}
        \centering
        \caption{Self harm related deaths}
        \label{Fig: selfHarmPredicted_splineVsRW2}
        \includegraphics[width=\linewidth]{selfHarmPredicted_splineVsRW2}
    \end{subfigure}
\end{figure}

\begin{table}[!h]
    \centering
    \caption{Model scores for the causes of suicide data. The First two rows are for alcohol related suicides and the latter two rows are for self harm related suicides. The columns are split into scores for estimation and the in-sample prediction.}
    \label{Tab: Suicide data model fit Scores}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{|c|c|ccc|ccc|}
        \hline
        \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Data\\ Scenario\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Model\\ Type\end{tabular}}} & \multicolumn{3}{c|}{\textbf{Estimation}} & \multicolumn{3}{c|}{\textbf{In-Sample Prediction}} \\ \cline{3-8} 
        &  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Interval Score}\\ $\pa{\times 10^{2}}$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Interval width}\\ $\pa{\times 10^{2}}$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{Coverage}\\ (\%)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Interval Score}\\ $\pa{\times 10^{2}}$\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Interval width}\\ $\pa{\times 10^{2}}$\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{Coverage}\\ (\%)\end{tabular} \\ \hline
        \multirow{2}{*}{\textbf{Alcohol}} & Spline& \multicolumn{1}{c|}{23.77} & \multicolumn{1}{c|}{23.77} & 100.00 & \multicolumn{1}{c|}{48.74} & \multicolumn{1}{c|}{48.74} & 100.00 \\ \cline{2-8} 
         & RW2 & \multicolumn{1}{c|}{27.16} & \multicolumn{1}{c|}{27.16} & 100.00 & \multicolumn{1}{c|}{104.03} & \multicolumn{1}{c|}{104.03} & 100.00 \\ \hline
        \multirow{2}{*}{\textbf{Self Harm}} & Spline & \multicolumn{1}{c|}{9.57} & \multicolumn{1}{c|}{9.57} & 100.00 & \multicolumn{1}{c|}{18.16} & \multicolumn{1}{c|}{18.16} & 100.00 \\ \cline{2-8} 
         & RW2 & \multicolumn{1}{c|}{10.97} & \multicolumn{1}{c|}{10.97} & 100.00 & \multicolumn{1}{c|}{36.04} & \multicolumn{1}{c|}{36.04} & 100.00 \\ \hline
    \end{tabular}%
    }
\end{table}

Figure \ref{Fig: PredictedLineplot} shows the observed, estimated and predicted log (incidence) rates of alcohol and self-harm related suicides by period and age. The biggest difference between the spline and RW2 estimates comes in the uncertainty bands for the predictions. The RW2 models bands are much wider than that of the splines.

\begin{sidewaysfigure}[!h]
    \centering
    \caption{Estimates and in-sample predicted values for the spline and random walk 2 models for alcohol (a) and self harm (b) related suicides. In each subfigure, The facets are for each of the age groups increasing from left-to-right and top-to-bottom. The $y$-axis is the log rate and the $x$-axis is the year. The green and blues solid lines are the fitted valued for the spline and random walk 2 models, respectively. The dashed lines are their associated $\alpha = 0.05$ uncertainty levels. The black dots are the true values and the vertical red dotted line is where the in-sample prediction starts.}
    \label{Fig: PredictedLineplot}
    \begin{subfigure}{.49\textwidth}
        \centering
        \caption{Alcohol related deaths}
        \label{Fig: alcoholPredictedLineplot}
        \includegraphics[width=\linewidth]{alcoholPredictedLineplot}
    \end{subfigure}%
    \begin{subfigure}{.49\textwidth}
        \centering
        \caption{Self harm related deaths}
        \label{Fig: selfHarmPredictedLineplot}
        \includegraphics[width=\linewidth]{selfHarmPredictedLineplot}
    \end{subfigure}
\end{sidewaysfigure}

\clearpage

\section{Discussion}

\begin{itemize}
    \item There is a theoretical link between smoothing splines and random processes
    \item Through a simulation study and example on mental health outcomes, we have shown this link holds for both estimation and prediction
    \item The biggest difference comes in uncertainty of predictions: the random processes uncertainty bands are much wider
    \item Since they are equivalent, the question an investigator has to ask themselves is what is more suitable: a frequestist analysis with smoothing splines, or a Bayesian analysis with random processes
    \begin{itemize}
        \item When to use frequestist
        \item When to use Bayesian
    \end{itemize}
    \item To demonstrate we used APC models
    \begin{itemize}
        \item Why: Because APC models have colinearity 
    \end{itemize}
    
    \item Mention alternatives for data with APC ({\color{violet} might fit better for the discussion section?})
    \begin{itemize}
        \item Age-period interaction
        \item Proxy cohort
        \item Lee-carter models
    \end{itemize}
\end{itemize}

==> documents/supplementaryMaterial.tex <==
\section{Spline basis functions}

Using a toy dataset defined by $A = 15$ ages and five knots, Figure \ref{Fig: differentBasisExamples} shows the examples the sets of bases defined by a cubic regression spline (CRS), B-spline (BS) and thin plate regression spline (TPRS). The bases are not orthogonalised to either an intercept or linear slope. 

\begin{figure}[!h]
    \centering
    \includegraphics[width=\linewidth]{differentBasisExamples}
    \caption{Examples of the basis functions for a cubic regression spline, B-spline and thin plate regression spline.}
    \label{Fig: differentBasisExamples}
\end{figure}

\clearpage

\section{Model scores from simulation study}

Table \ref{Tab: Simulation study model fit scores} shows the mean values for the model fit scores. These values correspond to the thick line within the `box' part of the box plots in the main manuscript. 

\begin{table}[!h]
    \centering
    \caption{Model scores for the simulation study. 
    %The first two columns define the model type and specifications. The next four columns are the model score, the Mean Absolute Error, Mean Square Error, Interval Score and (uncertainty) width. The top six columns are the results for estimation and the bottom six are for prediction.
    }
    \label{Tab: Simulation study model fit scores}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{cc|cccc}
        \hline
        \multicolumn{6}{c}{\textbf{Estimation} $\pa{\times 10^{-2}}$} \\
        \textbf{Model Type} & \textbf{Model Specification} & \textbf{Mean Absolute Error} & \textbf{Mean Square Error} & \textbf{Interval Score} & \textbf{Width} \\
        \hline
        \multirow{3}{*}{\textbf{Penalised Spline}} & CRS & 13.6459 & 3.0136 & 368.7563 & 10.8174 \\
         & BS & 13.6484 & 3.0144 & 369.5985 & 10.7644 \\
         & TPRS & 13.6511 & 3.0154 & 369.0794 & 10.8027 \\
        \hline
        \multirow{3}{*}{\textbf{Random Walk 2}} & U = 1 & 13.4897 & 2.9475 & 317.1453 & 14.2242 \\
         & U = 3 & 13.4848 & 2.9453 & 315.9283 & 14.3054 \\
         & U = 6 & 13.4833 & 2.9447 & 315.6193 & 14.3261 \\
        \hline
        \multicolumn{6}{c}{\textbf{Prediction} $\pa{\times 10^{-2}}$} \\
        \textbf{Model Type} & \textbf{Model Specification} & \textbf{Mean Absolute Error} & \textbf{Mean Square Error} & \textbf{Interval Score} & \textbf{Width} \\
        \hline
        \multirow{3}{*}{\textbf{Penalised Spline}} & CRS & 14.0717 & 3.1161 & 317.8736 & 16.0993 \\
         & BS & 14.0775 & 3.1187 & 316.8082 & 16.3022 \\
         & TPRS & 14.0690 & 3.1102 & 318.6231 & 15.9625 \\
        \hline
        \multirow{3}{*}{\textbf{Random Walk 2}} & U = 1 & 14.0885 & 3.1487 & 190.1655 & 32.0939 \\
         & U = 3 & 14.0915 & 3.1509 & 188.1159 & 32.5784 \\
         & U = 6 & 14.0930 & 3.1518 & 187.6254 & 32.6871 \\
        \hline
    \end{tabular}%
    }
\end{table}

\clearpage

\section{Heatmaps for complete data for mental health outcomes}

Figure \ref{Fig: ObservedHeatmap} shows heatmaps of deaths due to alcohol and self harm for the years 2006 -- 2021 and ages 10 -- 84. In the main analysis, we considered only the ages 25 -- 84 as there was a large difference between the ages 10 -- 24 and 25 -- 84. This is more notable for the self harm related deaths. 

\begin{figure}[!h]
    \centering
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{alcoholObservedHeatmap}
        \caption{Alcohol related deaths}
        \label{Fig: alcoholObservedHeatmap}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{selfHarmObservedHeatmap}
        \caption{Self harm related deaths}
        \label{Fig: selfHarmObservedHeatmap}
    \end{subfigure}
    \caption{Deaths due to alcohol and self harm for the years 2006 -- 2021 and ages 10 -- 84. Period is grouped into single years and operates along the $x$-axis. Age is grouped into five-year ages groups and operates along the $y-axis$. Cohort operates along the $y = x$ axis. Suicides are reported as log-rates with the dark-to-light colouring indicating lower-to-higher suicide rates.}
    \label{Fig: ObservedHeatmap}
\end{figure}

\clearpage

\section{Heatmaps from model fits of alcohol related deaths}

Figure \ref{Fig: alcoholPredictedHeatmap} shows the estimated and predicted values from the penalised spline and RW2 models for alcohol related deaths. The dashed red line indicates where the estimation ends and prediction starts.

\begin{figure}[!h]
    \centering
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{alcoholPredictedHeatmap_spline}
        \caption{Spline predictions}
        \label{Fig: alcoholPredictedHeatmap_spline}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{alcoholPredictedHeatmap_rw2}
        \caption{Random walk 2 predictions}
        \label{Fig: alcoholPredictedHeatmap_rw2}
    \end{subfigure}
    \caption{Estimates and predictions of deaths due to alcohol for the years 2006 -- 2021 and ages 25 -- 84. The left hand plot (a) is from the spline model and the right hand plot (b) is from the random walk 2 model.}
    \label{Fig: alcoholPredictedHeatmap}
\end{figure}

\clearpage

\section{Heatmaps from model fits of self harm related deaths}

Figure \ref{Fig: selfHarmPredictedHeatmap} shows the estimated and predicted values from the penalised spline and RW2 models for self-harm related deaths. The dashed red line indicates where the estimation ends and prediction starts.

\begin{figure}[!h]
    \centering
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{selfHarmPredictedHeatmap_spline}
        \caption{Spline predictions}
        \label{Fig: selfHarmPredictedHeatmap_spline}
    \end{subfigure}%
    \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=\linewidth]{selfHarmPredictedHeatmap_rw2}
        \caption{Random walk 2 predictions}
        \label{Fig: selfHarmPredictedHeatmap_rw2}
    \end{subfigure}
    \caption{Estimates and predictions of deaths due to self harm for the years 2006 -- 2021 and ages 25 -- 84. The left hand plot (a) is from the spline model and the right hand plot (b) is from the random walk 2 model.}
    \label{Fig: selfHarmPredictedHeatmap}
\end{figure}

\clearpage

\section{Spline and Random Walk Comparison Plots}

Figure \ref{Fig: Predicted_splineVsRW2} shows the estimated and predicted fitted values for the spline and RW2 models for both the alcohol and self harm related deaths. In each scenario, both sets of estimated and predicted values fall along the $y = x$ axis, hence are similar to one another.

\begin{figure}[!h]
    \centering
    \begin{subfigure}{.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{alcoholPredicted_splineVsRW2}
        \caption{Alcohol related deaths}
        \label{Fig: alcoholPredicted_splineVsRW2}
    \end{subfigure}%
    \begin{subfigure}{.49\textwidth}
        \centering
        \includegraphics[width=\linewidth]{selfHarmPredicted_splineVsRW2}
        \caption{Self harm related deaths}
        \label{Fig: selfHarmPredicted_splineVsRW2}
    \end{subfigure}
    \caption{Comparison of the estimated and in-sample predicted alcohol (a) and self harm (b) related suicide values from the spline and random walk 2 model. In each subfigure, the spline values are along the $x$-axis and the random walk 2 values are on the $y$-axis. The red dotted line is the $y=x$ axis. The green circles and blue triangles represent the estimated and predicted values, respectively.}
    \label{Fig: Predicted_splineVsRW2}
\end{figure}
